Seamless Integration of Analysis and Design: Automatic CAD Reconstruction of Post-Analysis Geometries

A key step during industrial design is the passing of design information from computer aided design (CAD) to analysis tools (CAE) and vice versa. Here, one is faced with a severe incompatibility in geometry representation: While CAD is usually based on surface representations, analysis mostly relies on volumetric representations. The forward pass, i.e., converting CAD data to computational meshes, is well understood and established. However, the same does not hold for the inverse direction, i.e., CAD reconstruction of deformed geometries resulting, e.g., from shape optimization. The few reconstruction methods reported mainly rely on spline fitting, in particular methods that rely on creating new splines simililar to shape reconstruction from 3D imaging. In contrast, this paper studies a novel approach that reuses the CAD data given in the initial design. We show that this concept leads to precise shape reconstructions while also preserving the initial notion of features defined during design. Furthermore, reusing the initial CAD representation reduces the shape reconstruction problem to a shape modification problem. We study this unique feature and show that it enables the reconstruction of CAD data from computational meshes by composing each spline in the initial CAD data with a single, global deformation spline. While post-processing is needed for use in current CAD software, this novel approach not only allows creating watertight models, but also enables reconstructing complete CAD models even from defeatured computational meshes.

==> input/sec_SplineFit.tex <==
\section{Shape reconstruction using individual spline fitting}
\label{sec_spline_fit}
\replaced{In this section, we describe how the deformed CAD representation can be reconstructed by fitting each geometric entity individually.
This can be necessary, if very small features need to be represented that are hard to resolve in a global context.
Even though fitting approaches are in general already available, what is novel here is to reuse the spline representations found in the initial CAD data.}
{The novelty in the presented approach is to reuse the spline representations found in the initial CAD data.
In this section, we apply this idea in the first of two developed methods: Reconstructing the deformed CAD representation by fitting each geometric entity individually.}\par
We will use the following notation: Again, $\initialmesh$ denotes the initial computational mesh,
and $\deformedmesh$ the deformed computational mesh, whereas $\spline{S}^i$ and $\deformed{\spline{S}}^i$ denote the $i$th spline in the geometry data in initial and deformed configuration.
Additionally, we denote by $\square\pointsonspline$ the subset of $\square$ which is interpolated by spline $\spline{S}$, where $\square$ is any set of nodes.\par 
Here, \textit{deformed} refers to the CAE results (Fig.~\ref{fig:problemStatement}(d)).
In our description, we do not distinguish explicitly between curves and surfaces, since all presented algorithms apply to curves and surfaces similarly if not explicitly stated otherwise. \par  
As indicated in Sec.~\ref{sec_splines}, the first step in spline fitting is to determine parametric coordinates $\boldsymbol{\Xi}$.
We utilize a linear variant of the projection algorithm by Hu and Wallner \cite{Hu2005}.
The actual spline fit then follows the exact approach described in Sec.~\ref{subsec_SF_intro}.
In the following, we thus focus on two aspects that arise specifically within this application: (1) How to refine the spline parameterization, and (2) how to deal with coarse computational meshes.\par
\added{The former aspect originates from that CAD representation parametrizes a surface or curve in the easiest way possible, e.g., four control points plus linear polynomials already describe a plane surface.
Suppose the target shape -- specifically its curvature -- significantly differs from the original shape, the paramtrization most likely cannot represent the new form, which
leads to an unsatisfactorily high remaining residual \eqref{eq:spline_fit_residual}. 
The flexibility of this parametrization needs to be increased by additional control points, 
}
\deleted{\eqref{eq:spline_fit_residual} remains unsatisfactorily high, the spline parameterization has to be refined}
 this can be achieved either by knot insertion or by degree elevation. \par
In view of maintaining smooth surfaces, we usually degree-elevate before inserting any new knots.
This choice comes with the disadvantage that some commercial CAD and CAE software can have trouble processing high-order splines.
For this reason, we choose to limit the resulting degree to four which still provides $G^2$ continuity, a common requirement in CAD.
If this degree increase does not yield the desired residual, additional knots have to be inserted.
For knot insertion, the algorithm has to decide in which parametric direction a knot has to be inserted and at which parametric coordinate.
Since each inserted knot adds several degrees of freedom to the optimization problem, , which enables the greatest further reduction of the residual should be chosen.
We achieve this using the procedure proposed by Weiss et al. \cite{WEISS200219}.
In a first step, this method determines the knot interval that shows the biggest residual and selects this element for knot insertion.
Subsequently, the exact new knot position is determined by weighting its proximity to existing knots against the current residual.
The complete procedure is detailed in Algorithm~\ref{alg:SplnFit}.
\begin{algorithm}[!h]
	\caption{Shape reconstruction by spline fit}\label{alg:SplnFit}
	\textbf{Input:} \\
	NURBS-only IGES file;\\
	Initial computational mesh $\initialmesh$;\\
	Deformed computational mesh $\deformedmesh$;\\
	\\
	\textbf{Output:} \\
	Updated IGES file;\\
	\\
	\textbf{Algorithm:} 
	\begin{algorithmic}[1]
		\State{$\Sigma = \left\{\spline{S}^i\right\} := \text{Collect all splines from IGES}$};
		\ForAll{$\spline{S}^i \in \Sigma$}
		\State \begin{varwidth}[t]{\linewidth}
			$\initialmesh\pointsonspline = \left\{\mathbf{x}_i \enskip \vert \enskip \norm{\mathbf{x}_i-\spline{S}^i}\leq \epsilon\right\} :=$ Collect all points which lay on the \\ spline $\spline{S}_i$;
			\end{varwidth}
		\State $ \text{Setup a mask} \enskip \Pi_i \enskip \text{s.th.} \enskip \initialmesh\pointsonspline = \Pi_i\initialmesh$;
		\State{\begin{varwidth}[t]{\linewidth}
			$\deformed{\spline{S}}^i = \spline{S}^i\text{.fit}\left(\initialmesh\pointsonspline=\Pi_i\initialmesh, \enskip \deformedmesh\pointsonspline=\Pi_i\deformedmesh\right)$ := \text{Apply Algorithm \ref{alg:SplnFit_standalone};}
			\end{varwidth}}
		\State Replace $\spline{S}^i$ by $\deformed{\spline{S}}^i$ in IGES file;
		\EndFor \\
		\Return Updated IGES file;
	\end{algorithmic}
\end{algorithm}
Here, we demand that (1) all mesh points lie within a small tolerance to the actual geometry, i.e., $\varepsilon \ll 1$, and (2) the portion of the computational mesh, which is fitted by each given spline, $\initialmesh_{\spline{S}}$, contains sufficiently many points.
The first condition needs to be fulfilled to robustly determine parametric coordinates.
However, it is also required to ensure that possibly remaining offsets between the initial geometry and $\initialmesh\pointsonspline$, which are, by design, reduced during the fitting procedure, do not yield unintended gaps between neighboring geometric entities after shape reconstruction.
The second condition must be fulfilled to yield a well-posed optimization problem.
However, in rare cases we observed that CAD data contains very small geometries whose dimension fall below the size of a single computational mesh element.
In such cases, additional sampling points can be added to $\initialmesh$, and -- by interpolation -- also to $\deformedmesh\pointsonspline$\replaced{, a step,}{ accordingly} which is described in detail in Sec.~\ref{subsec:interpolate_additional_data}.

\subsection{Interpolating additional points}
\label{subsec:interpolate_additional_data}
To obtain a well-posed, i.e., not under-determined system of equations, the number of grid points per parametric direction in $\initialmesh\pointsonspline$ needs to be equal or greater than the number of control points $\controlpoint$ in that parametric direction.
For numerical stability, we furthermore require that two nearby-located grid points may not be treated as different points when their distance falls below \num{1e-7}.
In rare cases, especially for curves, this criterion may be violated and additional points need to be generated.
In the following, we first present a criterion to determine whether additional data needs to be generated, before discussing two possible methods.\par 
To verify that no additional data is needed, we check two empirically derived conditions: (a) At least $l$ grid points $\mathbf{x}_i \in \initialmesh\pointsonspline$ must be located  in each non-zero knot span, where $l=1+\left(\max\left(0,\max\left(m_1-p,m_2-p\right)\right)\right)$.
Here, $p$ denotes the degree of the spline and $m_i$ refers to the multiplicities of the knot values that define this knot span.
This condition ensures that in areas of reduced continuity, target points are more densely populated.
(b) The total number of points in $\initialmesh\pointsonspline$ has to be greater or equal to the number of control points.\par
If any of the two conditions is not met, we construct new fitting data by sampling the spline at its \textit{Greville abscissae} computed as
\begin{equation}
	\bar{\xi}_a =\frac{1}{p} \sum_{i=1}^p{\xi_{a+i}}.
\end{equation}
We have found that using Greville abscissae provides the best approximation control with the fewest possible sampling points.\par 
While adding data to $\initialmesh\pointsonspline$ is straightforward, adding the corresponding data to $\deformedmesh\pointsonspline$ can be approached in several ways, two of which will be discussed here. \par
The first approach is based on the fact that a curve can be viewed as a surface boundary, which results in improved curve fitting and enhanced congruence between surfaces and their bounding curves:
Let a curve $\spline{C}$ be boundary to a surface $\spline{S}$.
Then, we determine the parametric coordinates $\boldsymbol{\eta}_{\text{add}}$ in the surface's parameter space, such that $\spline{S}\left(\boldsymbol{\eta}_{\text{add}}\right) = \spline{C}\left(\boldsymbol{\Xi}_{\text{add}}\right)$, where $\square_{\text{add}}$ denotes additional sampling data.
Particularly, $\boldsymbol{\Xi}_{\text{add}}$ are the curve's Greville abscissae.\par
Finally, points $\mathbf{x}_{\text{add}}$ are added to $\deformedmesh_{\spline{C}}$ by sampling the already reconstructed surface spline as $\mathbf{x}_{\text{add}}=\deformed{\spline{S}}\left(\boldsymbol{\eta}_{\text{add}}\right)$.
This approach strongly depends on successful surface reconstruction.
It's advantage, however, is that the resulting curves ensure a high level of watertightness since they follow their connected surfaces closely.
Since a single curve may bound multiple surfaces, for convenience, we sample the first connected surface found in the topology data's hierarchy tree.\par 
An alternative approach is to interpolate the computational mesh at additional \textit{ghost points}.
For the interpolation, we first determine the initial position of the new ghost point as $\mathbf{x}_{\text{add}} = \spline{C}\left(\boldsymbol{\Xi}_{\text{add}}\right)$.
Next, this point is expressed in terms of present mesh data and an offset vector:
Let $\mathbf{x}_{\star,i}$, $i\in[1,2,3]$ be the $i$th closest point to $\mathbf{x}_{\text{add}}$ in $\initialmesh_{\spline{C}}$.
Then, we define three vectors $\mathbf{d}_1 = \mathbf{x}_{\star,2} - \mathbf{x}_{\star,1}$,  $\mathbf{d}_3 = \mathbf{x}_{\star,3} - \mathbf{x}_{\star,1}$, and $\mathbf{d}_3 =\mathbf{d}_1 \times \mathbf{d}_2 $. 
Using these three vectors we can write
\begin{equation}
	\mathbf{x}_{\text{add}} =
	\underbrace{\begin{bmatrix}
		\vert & \vert& \vert  \\
		d_1   & d_2  & d_3  \\
		\vert & \vert& \vert 
	\end{bmatrix}}_{\mathbf{A}}
	\mathbf{b}.
	\label{eq:mesh_sampling}
\end{equation}
To generate additional data in the deformed computational grid, we then evaluate 
$\deformed{\mathbf{x}_{\text{add}}} = \deformed{\mathbf{A}} \mathbf{b}$, where 
$\deformed{\mathbf{A}}$ 
is constructed from the equivalent points in 
$\deformedmesh_{\spline{C}}$ to $\mathbf{x}_{\star}$ 
in 
$\initialmesh_{\spline{C}}$.\par 

\subsection{Example: Plate with hole}
\label{subsec:sf_results_plate}
As a first demonstration, we reconstruct CAD data for a generic plate \added{with dimensions $200 \times 100 \times 1.5$ and a central hole with diameter $50$}.
The geometry is built from six initially planar surfaces, cut by a two-piece cylinder in its center.
As for the remainder of this work, we plot all entities in the geometry data in individual color, to emphasize that we only change geometry data (cf. Fig.~\ref{fig:topology}).
The initial CAD representation is shown in Fig.~\ref{fig:res_sf_mesh_plate_initial}.\par
\begin{figure}[!h]
	\centering
	\includegraphics[width=.6\linewidth]{figures_results_SF_brep_initial_lochplatte.png}
	\caption{Initial geometry of plate with hole shown with different color for each entity in the geometry data. 
		Results will show the identical coloring for identical entities.
		The dimensions are $200\times100\times1.5$ and the hole diameter is $\num{50}$.}
	\label{fig:res_sf_mesh_plate_initial}
\end{figure}
For the reconstruction, a total of \num{3352} points in $\initialmesh$ is used.
The prescribed deformation is obtained from a mock simulation result and has no direct physical interpretation.
The maximal point deflection is $\num{18.88}$.\par
Using additional mesh sampling yields the result depicted in Fig.~\ref{fig:res_sf_plate} (a), while sampling from the previously reconstructed surfaces, yields the result shown in Fig.~\ref{fig:res_sf_plate} (b).
For this test case, visually indistinguishable results are obtained.

\begin{figure}[h]
	\centering
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt 
	\def \scale {0.7}
	\def \invariantscale {1/\scale}
	
		\scalebox{\scale}{  			
			\tikzset{every picture/.style={line width=0.75pt}} 
			
			\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
				\draw (130.27,389.96) node  {\includegraphics[width=193.67pt,height=96.83pt]{figures_results_SF_brep_sampled_from_mesh_lochplatte.png}};
				\node[scale=1/\scale, font=\normalsize, align=left] at (145,475) {(a)};				
				\draw (550.02,390.48) node  {\includegraphics[width=193.67pt,height=96.83pt]{figures_results_SF_brep_sampled_from_surface_lochplatte.png}};			
				\node[scale=1/\scale, font=\normalsize, align=left] at (545,475) {(b)};		
				\draw (341.74,267.44) node  {\includegraphics[width=193.67pt,height=96.83pt]{figures_problem_statement_grid_deformed.png}};
				\draw (340.83,163) node  	{\includegraphics[width=184.24pt,height=73.5pt]{figures_problem_statement_grid_undeformed.png}};
				\draw (340.71,59.5) node  	{\includegraphics[width=180.07pt,height=72.75pt]{figures_problem_statement_Geometry_undeformed_FreeCAD.png}};
							
				\draw [line width=0.75]    (340.18,203.64) -- (340.16,230.88) ;
				\draw [shift={(340.16,232.88)}, rotate = 270.05] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.8,-2.7) -- (0,0) -- (10.8,2.7) -- cycle    ;

				%Straight Lines [id:da0772615736788691] 
				\draw [line width=0.75]    (340.07,100.83) -- (339.92,120.38) ;
				\draw [shift={(339.91,122.38)}, rotate = 270.42] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.8,-2.7) -- (0,0) -- (10.8,2.7) -- cycle    ;
								
				% Modified arrows
				%Straight Lines [id:da7346244701793114]
				\draw [line width=0.75] [dash pattern={on 4.5pt off 4.5pt}] (458.88,56.25) -- (466.88,56.45) -- (464.88,296.02) -- (489.73,331.38) ;
				\draw [shift={(490.88,333.02)}, rotate = 234.9] [fill={rgb, 255:red, 0; green, 0; blue, 0 } ][line width=0.08] [draw opacity=0] (10.8,-2.7) -- (0,0) -- (10.8,2.7) -- cycle ;
				%Straight Lines [id:da6051598201724439]
				\draw [line width=0.75] [dash pattern={on 4.5pt off 4.5pt}] (225.88,54.45) -- (216.88,54.45) -- (216.88,296.02) -- (180.05,347.19) ;
				\draw [shift={(178.88,348.82)}, rotate = 305.74] [fill={rgb, 255:red, 0; green, 0; blue, 0 } ][line width=0.08] [draw opacity=0] (10.8,-2.7) -- (0,0) -- (10.8,2.7) -- cycle ;
				\draw [line width=0.75] (340.18,203.64) -- (340.16,230.88) ;
				\draw [shift={(340.16,232.88)}, rotate = 270.05] [fill={rgb, 255:red, 0; green, 0; blue, 0 } ][line width=0.08] [draw opacity=0] (10.8,-2.7) -- (0,0) -- (10.8,2.7) -- cycle ;
				\draw [line width=0.75] (340.07,100.83) -- (339.92,120.38) ;
				\draw [shift={(339.91,122.38)}, rotate = 270.42] [fill={rgb, 255:red, 0; green, 0; blue, 0 } ][line width=0.08] [draw opacity=0] (10.8,-2.7) -- (0,0) -- (10.8,2.7) -- cycle ;
				%Straight Lines [id:da7597059080408273]
				\draw [line width=0.75] (231.27,296.02) -- (187.13,351.45) ;
				\draw [shift={(185.88,353.02)}, rotate = 308.53] [fill={rgb, 255:red, 0; green, 0; blue, 0 } ][line width=0.08] [draw opacity=0] (10.8,-2.7) -- (0,0) -- (10.8,2.7) -- cycle ;
				%Straight Lines [id:da4468354284841405]
				\draw [line width=0.75] (450.5,296.02) -- (482.64,336.45) ;
				\draw [shift={(483.88,338.02)}, rotate = 231.52] [fill={rgb, 255:red, 0; green, 0; blue, 0 } ][line width=0.08] [draw opacity=0] (10.8,-2.7) -- (0,0) -- (10.8,2.7) -- cycle ;
								
				\draw (475,51) node [draw=black, anchor=north west][inner sep=2.5pt]   [align=center] {
						Initial CAD representation
					};
				% Text Node
				\draw (473,156) node [draw=black, anchor=north west][inner sep=2.5pt]   [align=center] {
					Initial computational mesh
				};
				\draw (474,239) node [draw=black, anchor=north west][inner sep=2.5pt]   [align=center] {
							Shape-optimized \\
							computational mesh
							};								% Text Node
				\draw(270, 359) node [draw=black, anchor=north west][inner sep=2.5pt]   [align=center] {
					Reconstructed  \\ CAD representation
					};
			\end{tikzpicture}
		}
		
		\caption{(a) Reconstructed shape using additional point sampling utilizing formula \eqref{eq:mesh_sampling}. (b) Reconstructed shape using additional point sampling from previously deformed surfaces.
		Both variants yield \deleted{equally well} CAD reconstructions \added{of equal quality}.
		} 
		\label{fig:res_sf_plate}
\end{figure} 

\subsection{Example: Sensor box}
\label{subsec:sf_results_sensor}
As a second and both computationally and methodologically more challenging example, we reconstruct CAD data for a pressure sensor box.
The initial geometry has length, width and depth of $\mathcal{O}\left(10\right)$ and is shown in Fig.~\ref{fig:res_sf_mesh_sensor_initial}.

\begin{figure}[h]
	\centering
	\includegraphics[width=.5\linewidth]{figures_results_SF_brep_initial_sensor.png}
	\caption{Initial sensor box shown with different color for each entity in the geometry data. Results will show the identical coloring for identical entities.}
	\label{fig:res_sf_mesh_sensor_initial}
\end{figure}
For the reconstruction, a total of $26177$ grid points is used.
In absence of simulation data, we prescribe a non-linear deformation as nodal offsets $\mathbf{d}_j$ for all $\mathbf{x}_j \in \initialmesh$  with $c=0.15$ via:
\begingroup
\allowdisplaybreaks[0]
\begin{subequations}\label{eq:prescribed_deformation_sensor}
	\begin{alignat}{3}
		\mathbf{x}_{\mathrm{center}} &= \mybar{0.6}{1pt}{\initialmesh}\\
		\mathbf{r} &= \left\{r_j \enskip \big\vert \enskip r_j = \left(\mathbf{x}_j-\mathbf{x}_{\mathrm{center}}\right)^2\right\}\\
		\mathbf{d}_j &= c \frac{r_j}{\underset{j}{\max\,}{r_j}}\left(\mathbf{x}_j-\mathbf{x}_{\mathrm{center}}\right),
	\end{alignat}
\end{subequations}
\endgroup
which yields a maximum point deflection of $6.59$ and an average deflection of $1.70$.
Using sampling from the mesh yields the result depicted in Fig.~\ref{fig:res_sf_mesh_sensor}, while sampling from the previously reconstructed surfaces, yields the result shown in Fig.~\ref{fig:res_sf_surface_sensor}.

\def \subfigwidth {.45\linewidth}
\begin{figure}[hb]
	\centering
	\begin{subfigure}[t]{\subfigwidth}
		\centering
		\includegraphics[width=.9\textwidth]{figures_results_SF_brep_sampled_from_mesh_PressureSensor.png}
		\caption{Reconstructed shape using additional point sampling utilizing formula \eqref{eq:mesh_sampling}.}
		\label{fig:res_sf_mesh_sensor}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{\subfigwidth}
		\centering
		\includegraphics[width=.9\textwidth]{figures_results_SF_brep_sampled_from_surface_PressureSensor.png}
		\caption{Reconstructed shape using additional point sampling from previously deformed surfaces.}
		\label{fig:res_sf_surface_sensor}
	\end{subfigure}
	\caption{Reconstructed shapes using additional point sampling from mesh and connected surfaces.}
	\label{fig:res_sf_sensor}
\end{figure}
As the Figures \ref{fig:res_sf_plate} and \ref{fig:res_sf_sensor} reveal, both sampling options yield satisfactory results and high quality CAD data.
The difference between the two sampling methods is hardly noticeable.
A close look, presented in Fig.~\ref{fig:res_sf_comparison_sampling}, suggests that surface sampling leads to even smoother surface reconstructions.
Thus, the practitioner may prefer surface sampling compared to the mesh sampling based on Eq.~\eqref{eq:mesh_sampling}.
Using mesh sampling, we obtain a point wise maximum error of $\num{2.52e-2}$ for the plate with a hole and $\num{3.53e-2}$ for the pressure sensor.
Using sampling from the surface, we respectively obtain $\num{2.52e-2}$ for the the plate with a hole and $\num{2.82e-2}$ for the pressure sensor.
\replaced{Note, however, that these numbers depend on the chosen optimization settings and only give a rough comparison of the two approaches. }
{ We shall mention that these are, however, rather qualitative numbers since the achievable accuracy depends on the chosen optimization settings.}\par

\def \subfigwidth {.45\linewidth}
\begin{figure}[h]
	\centering
	\begin{subfigure}[t]{\subfigwidth}
		\centering		
		\tikzset{every picture/.style={line width=0.75pt}}       
		\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
			\draw (125.52,152.5) node  {\includegraphics[trim={0 0 0 8cm}, clip, width=0.4\linewidth]{figures_results_SF_brep_sampling_comp2_technikum_fromMesh.png}};
			\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=0.74 ][line width=1.5] (134,122) ellipse (0.4cm  and 0.25cm);		
		\end{tikzpicture}
		\subcaption{Detailed view on a trimming line reconstructed using sampling from the mesh, c.f. Fig.~\ref{fig:res_sf_mesh_sensor}.
		Insufficient recovery marked in red.}
		\label{fig:res_sf_mesh_sensor_detail}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{\subfigwidth}
		\centering
		\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
			\draw (125.52,152.5) node  {\includegraphics[trim={0 0 0 8cm}, clip, width=0.4\linewidth]{figures_results_SF_brep_sampling_comp2_technikum_surfSample.png}};		
		\end{tikzpicture}
		\subcaption{Detailed view on a trimming line reconstructed using sampling from previously fitted surfaces, c.f. Fig.~\ref{fig:res_sf_surface_sensor}.}
		\label{fig:res_sf_surfaces_sensor_detail}
	\end{subfigure}
	\caption{Detailed comparison between sampling additional data from the mesh using Eq.~\eqref{eq:mesh_sampling} (left) and sampling from previously reconstructed surfaces (right).
	We exemplary show the back view of the pressure fitting.
	The detailed view, however, underpins the fact that we can hardly detect any differences.}
	\label{fig:res_sf_comparison_sampling}
\end{figure}
